Studies on the response of a water-Cherenkov detector of the Pierre Auger Observatory to atmospheric muons using an RPC hodoscope

Extensive air showers, originating from ultra-high energy cosmic rays, have been successfully measured through the use of arrays of water-Cherenkov detectors (WCDs). Sophisticated analyses exploiting WCD data have made it possible to demonstrate that shower simulations, based on different hadronic-interaction models, cannot reproduce the observed number of muons at the ground. The accurate knowledge of the WCD response to muons is paramount in establishing the exact level of this discrepancy. In this work, we report on a study of the response of a WCD of the Pierre Auger Observatory to atmospheric muons performed with a hodoscope made of resistive plate chambers (RPCs), enabling us to select and reconstruct nearly 600 thousand single muon trajectories with zenith angles ranging from 0$^\circ$ to 55$^\circ$. Comparison of distributions of key observables between the hodoscope data and the predictions of dedicated simulations allows us to demonstrate the accuracy of the latter at a level of 2%. As the WCD calibration is based on its response to atmospheric muons, the hodoscope data are also exploited to show the long-term stability of the procedure.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 1342 2019-01-29 17:20:57Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard *.sty *.bib figs/*) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := /bin/bash
PDFS := $(addsuffix .pdf, $(TARGETS))

ifeq (, $(shell which latexmk))
  LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)
  # 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
  COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'
  define basic_latex_rule
    for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
  endef
  ifeq ($(USEBIBTEX), 1)
    define latex_rule
      $(LATEX) $< ; bibtex $*
      $(call basic_latex_rule)
    endef
  else
    define latex_rule
      $(call basic_latex_rule)
    endef
  endif
else
  define latex_rule
    latexmk $(if $(filter 1, $(USEPDFLATEX)), -pdf, ) $<
  endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,.maf,.fff,.lot,.ttt,.bcf,.run.xml,.fdb_latexmk,.fls,.synctex.gz}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

